Multilingual Sentence-Level Semantic Search using Meta-Distillation Learning

Multilingual semantic search is the task of retrieving relevant contents to a query expressed in different language combinations. This requires a better semantic understanding of the user's intent and its contextual meaning. Multilingual semantic search is less explored and more challenging than its monolingual or bilingual counterparts, due to the lack of multilingual parallel resources for this task and the need to circumvent "language bias". In this work, we propose an alignment approach: MAML-Align, specifically for low-resource scenarios. Our approach leverages meta-distillation learning based on MAML, an optimization-based Model-Agnostic Meta-Learner. MAML-Align distills knowledge from a Teacher meta-transfer model T-MAML, specialized in transferring from monolingual to bilingual semantic search, to a Student model S-MAML, which meta-transfers from bilingual to multilingual semantic search. To the best of our knowledge, we are the first to extend meta-distillation to a multilingual search application. Our empirical results show that on top of a strong baseline based on sentence transformers, our meta-distillation approach boosts the gains provided by MAML and significantly outperforms naive fine-tuning methods. Furthermore, multilingual meta-distillation learning improves generalization even to unseen languages.

==> algorithms/inner-loop-eval.tex <==
\begin{algorithm}[t!]
\caption{INNER\_LOOP$_{\mbox{\tiny{eval}}}$
}
\begin{small}
\begin{algorithmic}[1]

% \textbf{Function} {INNER\_LOOP}($\mathcal{T}$, $\theta$, $\alpha$, $n$)%\textbf{Function} {INNER\_LOOP}($\mathcal{T}$, $\theta$, $\alpha$, $n$)


\Function{INNER\_LOOP}{$\mathcal{T}$, $\theta$, $\alpha$, $n$}
   \FOR{each $T_j = (S_j^{X}, Q_j^{\xprime{X}})$ in $\mathcal{T}$}
    \STATE Initialize $\theta_{j} \leftarrow \theta$ 
    \FOR{$t=1\ldots n$}
    \STATE Evaluate $\partial B_{\theta_{j}} / \partial \theta_{j}  = \nabla_{\theta_{j}} \mathcal{L}^{S_j^X}_{T_{j}}(B_{\theta_{j}})$
    \STATE Update $\theta_{j} = \theta_{j} - \alpha \partial B_{\theta_{j}} / \partial \theta_{j} $
    
    \ENDFOR
    
    \STATE $\mathcal{L_{avg}}^{S_j^{\xprime{X}}}_{T_j}(B_{\theta_{j}})$ =
    \STATE Evaluate query loss $\mathcal{L}^{Q_j^{\xprime{X}}}_{T_j}(B_{\theta_{j}}) $ and save it for knowledge distillation and outer loop
    \ENDFOR
\EndFunction
\end{algorithmic}
\end{small}
\label{procedure-inner-loop-eval}
\end{algorithm}

==> figures/base_models.tex <==
% \begin{figure*}[t]
%     \begin{subfigure}[b]{0.7\textwidth}
%         \centering
%         \includegraphics[width=1\textwidth]{images/dualencodertripletloss-Page-5.pdf}
%         \caption{Asymmetric Semantic Search: Retrieval-based Question Answering.}
%         \label{fig:basemodel-asym}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.4\textwidth}
%         \includegraphics[width=1\textwidth]{images/BaseModelSym.pdf}
%          \caption{Symmetric Semantic Search: Semantic Similarity.}
%         \label{fig:basemodel-sym}
%      \end{subfigure}
%  \caption{\label{fig:base-model} Architecture of Transformer-based triplet encoder for asymmetric question span-based semantic search and dual-encoder for symmetric semantic search.}
% \end{figure*}

\begin{figure*}[ht]
\centering
\includegraphics[width=0.7\textwidth]{images/dualencodertripletloss-Page-3.drawio.pdf}
\caption{\label{fig:base-model} Architecture of Transformer-based triplet encoder for asymmetric question span-based semantic search and dual-encoder for symmetric semantic search.}
\end{figure*}

==> figures/conf_matrices.tex <==
\begin{figure*}[t]
    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{images/sbertconfmat.png}
        \caption{MAP@20 of S-BERT Base.}
        \label{fig:s-bert-x-conf-mat-base}
    \end{subfigure}
    \begin{subfigure}[b]{0.5\textwidth}
        \includegraphics[width=1\textwidth]{images/mamlconfmat.png}
         \caption{MAP@20 of \maml{}.}
        \label{fig:s-bert-x-conf-mat-maml}
     \end{subfigure}
 \caption{Confusion matrices comparing monolingual/cross-lingual performances of the base model vs T-MAML.}
 \label{fig:x-mono-confusion-matrices}
\end{figure*}

==> sections/relatedwork_v2.tex <==
\section{Related Work}

One popular approach to bilingual semantic search is to reduce the task to monolingual semantic search by using machine translation~\cite{lu-querytrans-aclclp08,nguyen-wikiTranslate-clef08,jones-domainspecificquery-ijcnlp08}. However, such systems often suffer from error propagation and overheads from API calls rendering them inefficient for multilingual semantic search, as the number of language combinations in the query and content to be retrieved can get prohibitively large~\cite{Savoy2019}. Pre-trained multilingual transformer-based models such as \mbert{}~\cite{bert-devlin-naacl19} and \xlmr{}~\cite{conneau-etal-2020-unsupervised} have been used as off-the-shelf encoders in multilingual semantic search, however their performance, especially for ad-hoc semantic search, is still lacking~\cite{litschko-multienc-infretr2022}. Knowledge distillation, which is leveraged to improve the alignment between languages~\cite{reimers-gurevych-2020-making}, still yields mixed results, under-performing machine translation on some language pairs and the teacher model is often fixed and not flexible enough to adapt to the student's capacity~\cite{zhou-bertlearns2teach-acl22}. Contrastive-distillation learning, which is a new hybrid form of low-resource learning, has been used to produce higher-quality multilingual distillation-based sentence representations~\cite{tan-multicontrastive-eacl23}. However, their approach still relies on medium-scaled data including monolingual corpora and back-translation. %  In our work, we investigate other ways to further improve the transfer between different languages on top of semantic specialization in a data-efficient manner. 

% Maybe also group with the previous paragraph: Cross-lingual Meta-transfer learning and its gains 
%% talk about cross-lingual meta-transfer learning in general
%% talk about multilingual meta-transfer learning and how it is under-explored
%% shortcomings to your current approach

% % Group this paragraph with the latter paragraph: Shortcomings of meta-transfer learning and knowledge distillation and how combining them could help 
Meta-transfer learning, or ``learning to learn'' has found favor in cross-lingual transfer learning for numerous downstream applications~\cite{DBLP:conf/emnlp/GuWCLC18,DBLP:conf/icassp/HsuCL20,DBLP:conf/acl/WinataCLLXF20, DBLP:conf/interspeech/ChenHLL20, DBLP:conf/aaai/XiaoGZZLL21,nooralahzadeh-etal-2020-zero,mhamdi-etal-2021-x}. For retrieval tasks, its application has been restricted to the monolingual case~\cite{lin-chen-2020-preliminary,laadan2019rankml,carvalho2008meta}. More recently, meta-transfer learning has been extended multilingually by exploring joint multi-task and multi-lingual transfer~\cite{tarunesh-metamulti-acl21,van2021multilingual}. Meta-learning has also been leveraged to improve the performance of knowledge distillation by consolidating the feedback loop between the teacher and student networks to help the teacher transfer better to the student~\cite{zhou-bertlearns2teach-acl22, liu-metakd-arxiv22}. Inversely, knowledge distillation has been leveraged to improve meta-learning, especially MAML~\cite{maml-finn-icml17} by making it more portable~\cite{zhang-kdf4maml-ecai20}. To the best of our knowledge, we are the first to adapt multilingual meta-transfer learning and to extend an approach based on meta-distillation to multilingual semantic search and to a multilingual application in general.

==> table/tab_multi-baselines-transfermodes.tex <==
\begin{table*}[ht!] 
\centering
\scalebox{0.75}{
\begin{tabular}{l|l|llllll} \toprule 
\textbf{Model} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{Sampling} \\ \textbf{Mode}\end{tabular}} & \multicolumn{5}{c}{\textbf{Testing Transfer Modes}}  \\
& & \monomono{} &  \monobil{} &  \monomulti{} & \bilmulti{} & \mixt{} & \trans{} \\ 
\midrule 
\multirow{2}{*}{\sbert{}+\finetune{}^{*}} & sim & 29.3 \small{$\pm$ 9.0} & 31.1 \small{$\pm$ 3.4} & 22.6 \small{$\pm$ 5.2} & 25.1 \small{$\pm$ 4.0} & 23.7 \small{$\pm$ 5.9} & 22.3 \small{$\pm$ 9.5}  \\
& rand & 34.3 \small{$\pm$ 2.9} & 36.7 \small{$\pm$ 3.5} & 20.1 \small{$\pm$ 7.7} & 14.1 \small{$\pm$ 6.5} & 27.7 \small{$\pm$ 4.6} & 30.3 \small{$\pm$ 3.4} \\
\cline{2-8}
\multirow{2}{*}{\sbert{}+\maml{}^{*}}  & sim & 51.9 \small{$\pm$ 2.0} & 52.5 \small{$\pm$ 2.0} & 48.0 \small{$\pm$ 3.8} & 48.1 \small{$\pm$ 3.3} & 49.6 \small{$\pm$ 1.9} & 49.2 \small{$\pm$ 1.7} \\
& rand &  52.1 \small{$\pm$ 2.2} & 52.4 \small{$\pm$ 3.1}  & 51.6 \small{$\pm$ 1.9} & 51.0 \small{$\pm$ 2.3}  & 50.3 \small{$\pm$ 3.2}  & 50.6 \small{$\pm$ 3.2}  \\
\bottomrule
\end{tabular}
}
\caption{\label{tab:multi-baselines-transfermodes} Multilingual performance in terms of \map{} tested for different transfer modes (using the test portion of \lareqa{}). * denotes best model version. Best results for each base model are highlighted in \textbf{bold}, whereas best results across base models are \underline{underlined} too and best results across transfer modes are \textit{italicized}.}
\end{table*}

==> table/tab_multi-negsampling.tex <==
\begin{table*}[t] 
\centering
\scalebox{0.90}{ 
\begin{tabular}{l|lllllllll} \toprule 
\multicolumn{8}{c}{\textbf{Testing Languages}}  \\
Sampling Mode & AR &  DE &  EL & HI & RU & TH & TR & Mean \\ 
\midrule 
random & \textbf{41.10} & \textbf{49.88} & \textbf{48.32} & \textbf{48.22} & \textbf{50.49} & 47.02 & \textbf{48.86} & \textbf{47.70} \\
hard & 38.32 & 48.94 & 46.59 & 44.76 & 47.84 & 46.64 & 47.44 & 45.79 \\
semi-hard & 39.09 & 49.44 & 47.33 & 45.95 & 48.67 & \textbf{47.30} & 48.03 & 46.54 \\
% easy & \multicolumn{8}{c}{IN PROGRESS}   \\
% hybrid & \multicolumn{8}{c}{IN PROGRESS} \\
\bottomrule
\end{tabular}
}
\caption{\label{tab:multi-negsampling} Multilingual performance in terms of \map{} tested for different languages (using the test portion of \lareqa{}) using \maml{} for \monomulti{} mode.}
\end{table*}
